Larimar: Large Language Models with Episodic Memory Control

Efficient and accurate updating of knowledge stored in Large Language Models (LLMs) is one of the most pressing research challenges today. This paper presents Larimar - a novel, brain-inspired architecture for enhancing LLMs with a distributed episodic memory. Larimar's memory allows for dynamic, one-shot updates of knowledge without the need for computationally expensive re-training or fine-tuning. Experimental results on multiple fact editing benchmarks demonstrate that Larimar attains accuracy comparable to most competitive baselines, even in the challenging sequential editing setup, but also excels in speed - yielding speed-ups of 8-10x depending on the base LLM - as well as flexibility due to the proposed architecture being simple, LLM-agnostic, and hence general. We further provide mechanisms for selective fact forgetting, information leakage prevention, and input context length generalization with Larimar and show their effectiveness. Our code is available at https://github.com/IBM/larimar

==> sections/introduction.tex <==
\section{Introduction}

 Pre-trained Large Language Models have achieved impressive performance on various Natural Language Processing (NLP) tasks~\citep{devlin2018bert,raffel2020exploring,brown2020language,vaswani2017attention}, and are often considered as knowledge repositories \cite{}. However, there remain challenges to be resolved to keep such models relevant, safe, and ethical after they have been deployed -- so their knowledge needs to be constantly updated.% One  prevalent challenge is generalization to long-form information beyond   the input length limit.  Another important challenge is  editing and unlearning of LLM's knowledge, %knowledge update 
 It is critical to develop efficient mechanisms for knowledge editing and forgetting  
 so that models can protect privacy, eliminate bias and hallucination, and catch up with time-sensitive facts. Roughly speaking, when an LLM generates text composed of undesired, incorrect, or obsolete facts, model editing should remove the wrong fact from the LLM's ``memory", and optionally replace it with the desired outcome.  
 Optionally, the model editing should satisfy three key desiderata: (i) \emph{locality}, ensuring that the model performance does not degrade elsewhere that is unrelated to edits;  (ii) \emph{generality}, ensuring that the model behaves similarly when presented with an edit reformulation; (iii) \emph{speed/scalabilty}, which is important in both sequential and batch editing situations.  

 

% Numerous approaches have been proposed that broadly fall into three main categories~\citep{yao2023editing} : 'Cache-based', 'Meta-learning' and 'Locate and Edit'.  Alternatively, \url{https://arxiv.org/pdf/2401.01286.pdf} uses Recognition Phase, Association Phase and Mastery Phase to classify the various methods. 
%\question{Shall we go with  Recognition Phase, Association Phase and Mastery Phase then? and mention in the end that an alternative classifiction is that of ~\citep{yao2023editing} : 'Cache-based', 'Meta-learning' and 'Locate and Edit' ?}

Numerous editing approaches have been proposed; for  comprehensive surveys on model editing methods, see \cite{yao2023editing, zhang2024comprehensive, wang2023knowledge}. Editing methods broadly fall into three categories:  'Recognition Phase', 'Association Phase' and 'Mastery Phase'. ~\citep{zhang2024comprehensive}. This classification essentially accounts for whether or not the  base model's parameters are affected. ~\footnote{Note that  an alternative classification is that of ~\citep{yao2023editing} : 'Cache-based', 'Meta-learning' and 'Locate and Edit'.}. 
%  The success of knowledge editing is usually evaluated along three dimensions (Yao et al., 2023; De Cao et al., 2021; Meng et al., 2022a,b) - (i) reliability, which measures if the post-edit model accurately recalls the newly edited fact, (ii) generalization, which measures if the post-edit model accurately recalls the newly edited facts for different phrasings of the edited fact, and (iii) locality (also known as specificity (Meng et al., 2022a,b)), which measures if the edited fact changes unrelated or neighboring facts.
 While current model editing methods have demonstrated significant  promise \citep{yao2023editing}, they do come with certain shortcomings. Existing editing methods mostly rely on either training  or  locally updating the parameters of the base model (or some auxilary model) on an edit dataset, and generalize well  within this seen distribution. However, they are less capable of systematic generalization to edits drawn from unseen  distributions, which affects their scalability due to increased cost and speed -  issues that are critical for fixing deployed models in real-world.   % Requirement of  edit-specific training or tracing and update, and therefore lacks generalization towards new/unrelated edits. This issue further leads to reduced speed and higher cost of edits.
 Further,  it has been reported that fact-specific knowledge within LLM is not as localized as it is believed to be \cite{hase2023does}, therefore local parameter update may not be sufficient to fully enforce the knowledge edit.  At the same time, even locally updating LLM's parameters can cause performance degradation on other tasks \cite{}. %  they are believed to be,  leading to the leakage of information \cite{hase2023does}. On the other hand, recent works reveal that  from causal tracing methods may not correlate with edit performance \cite{hase2023does}  (iii)  
 The editing task becomes more challenging, when multiple edits are needed to be made to the model %Performance evaluation is mostly done on  when only a single edit is made to the model. It has been found that making multiple edits, 
  either in a sequential or in a batched manner, former being more realistic. Several recent works report failure of existing editing methods in those situations,  leading to significant performance degradation of the LLM (Mitchell et al., 2021, 2022; Meng et al., 2022b) \cite{gupta2024model, li2023unveiling, gu2024model}, revealing  forgetting of the older edits, causing innate knowledge distortion,  enhancing inherent knowledge inconsistencies, or loss of general abilities in LLMs. A number of external cache/memory/codebook-based editing methods have been proposed to tackle those challenges, where base model is not directly edited. However, computational efficiency in terms of writing in and reading from those slot-based memories remains to be an issue.  %Methods such as GRACE  focus on solving some of these issues \PD{how?}; however, they still require edit-specific finetuning and edits are only done at a specific layer.  %(iv) The neighborhood specificity in current editing methods appears to lack robustness \cite{hoelscher2023detecting} \PD{shall we mention as ours is no better}. 
Last but not the least, 
selective knowledge forgetting remains challenging for current model editing methods, as suggested in \cite{ishibashi2023knowledge}

 
  
%The above methods require either model training (finetuning, metalearning) or tracing plus parameter update specific to  edit datasets. 
%\question{Carefully check the validity of the issues below.}
%The main issues with the above methods is that 
%\begin{itemize}
    %\item knowledge editing and unlearning - is needed after model deployed. important for keeping the model relevant, safe, and ethical. 
   % \item quick addressing is important in both sequential and batch editing situations.
    %\item important to ensure model performance does not degrade elsewhere that is unrelated to edits.
%They do not \emph{generalize} well beyond. The methods are not effective in \emph{fact forgetting}.  Existing methods are not \emph{fast enough} to perform real-time editing. They cannot maintain performance on the original data, or show edit efficiency that is robust when multiple edits are performed in a sequential manner.

%In this paper, we tackle these issues and propose Larimar, a novel architecture coupling generative LLM architectures with generative associative memory modules.  





%Building knowledge of the world over time and acting on it requires the ability to receive activity patterns from sensory neurons, encode them into new information, store that information long-term, selectively integrate it into our existing knowledge structures, retrieve that information, and deploy it when needed.

%LLMs currently do not possess ability to explicitly encode information and ``form memories'' of their recent past. Yet, doing so is critical to performing tasks that demand long-term dependencies, such as hallucination prevention, reasoning, generalization, continual learning, and value alignment.

%The Complementary Learning Systems (CLS) framework suggests that the brain achieves these complex feats through a division of labor across more than one interacting system, for example between the neocortex and hippocampus. The neocortex acts as a probabilistic generative model, which interacts with the world and maintains a semantic representation of it, whereas the hippocampus retains recent (episodic) memories, gradually consolidates them into longer-term ones, and is involved in the retrieval of memories.
%\paragraph{Core Idea.} %Our Larimar architecture is inspired by the interactions between neocortex and hippocampus in the brain, which are bi-directional and autonomous in nature. Those interactions promote teaching neocortex new information over time, as well as memory consolidation. 

%Larimar is a family of neural architectures with memory, inspired by the efficient information capture, storage, and retrieval processes in biological brains. 

To address above-mentioned challenges, our approach here is to construct Larimar -- a class of generative LLM (GLM) architectures augmented with and controlled by an external associative memory module $M$ that is distributed and generative. For real-time knowledge editing, we aim to dynamically update $M$.  The Larimar framework is loosely inspired from the  complementary learning systems (CLS) theory \cite{kumaran2016learning}, which provides rationale for coupling complementary fast (hippocampus) and slow (neocortex) memory systems in brain. In CLS theory,  an integrated learning system comprised of different dedicated subsystems outperforms either subsystem. E.g.,  neocortex-hippocampus interactions in brain is known to promote adaptive behavior via memorization and generalization \cite{sun2023organizing}. Further, it is proposed that the memory consolidation  from hippocampus to neocortex is facilitated  through the activation synchronized with multiple exact or false replays of the encoded experience in hippocampus -- suggesting the hippocampus  taking the form of a generative associative network \cite{ramirez2013creating}. 

To pursue this view, we build Larimar framework by seeking to the sparse distributed memory (SDM) model proposed by Kanerva \citep{kanerva1988sparse}, which  decouples the memory capacity  from the input dimensionality  by introducing a fixed-size distributed memory store (as opposed to slot-based memories).  Recent works have extended original SDM model to  a hierarchical conditional generative memory model \citep{wu2018kanerva}, referred as Kanerva Machines (KM), which combines  slow-learning neural networks (like RNN)  with a fast-adapting memory. Memory is treated as a global latent variable for an episode of input samples. The memory writes and reads are interpreted as inference in a generative model, wherein memory is now treated as a distribution, $p(M)$. %which combines  slow-learning neural networks with a fast-adapting linear Gaussian model as memory. In this framework, named as Generative Kanerva Machines ,  memory writes and reads are interpreted as inference in a generative model, wherein memory is now treated as a distribution, $p(M)$. 
The model learns to compress an episode of samples  through  learnable addresses and  a learned memory-dependent prior. 
As a  linear gaussian model of memory is used in Kanerva Machines, once the model  is meta-learned via end-to-end gradient descent, the posterior memory remains analytically tractable. Therefore, the posterior memory parameters can be  updated using Bayesian update (or equivalent) rule, enabling fast write when a new data episode arrives. %More recently, Pham, et al., have proposed a more efficient one-shot memory update by solving a minimization problem \cite{pham2021generative} that is equivalent to Bayesian update. This minimization problem, which corresponds to solving a linear system of equations, is efficiently done via computing matrix pseudo inverses. 

%In this work, we adapt  particularly to  the one-shot memory update approach proposed by \cite{gpm}. %In Kanerva machine also applies conjugate normal-normal Bayesian update to adapt its top level memory matrix once the model is meta-learned via end-to-end gradient descent
 Inspired by this line of works, we end-to-end train an external generative associative memory module $M$ together with a GLM $d$. The goal is to achieve a  hierarchical conditional generative model,  such that (i) $M$ is a global latent variable for $X$, an episode consisting of $N$ facts, (ii) readout from $M$ is used by the decoder to reconstruct input $X$, and (iii) posterior of M can undergo fast and dynamic update by  Bayesian update. This dynamic updating mechanism of memory together with the memory-augmented decoding enables Larimar to handle unseen edits in a training-free manner,  which is not the case for existing editing methods. We demonstrate Larimar on single fact, sequential and batch editing tasks. We further demonstrate a training-free  selective forgetting operation in Larimar based on one-shot memory updating mechanism.
 
  Previous works on generative memory models %, and more generally, associative memory models,
  have tested model's performance mostly on image reconstruction, denoising, and generation tasks. To our knowledge, this is the first work that proposes that trains a hierarchical conditional generative memory model for language and tackle LLM editing in a more bio-inspired manner via dynamically updating the generative distributed memory.   % the memory module is a faster and more dynamic learner than the GLM.  The resulting generative memory module is fixed-size and is fast to write in an episode of n facts and read out the same.   The read/write operations in Larimar are formalized as seeking robust solutions of linear systems and leveraging matrix pseudo-inverses, which is inspired by the recent work by \cite{gpm}. The end-to-end training ensures that the language modeling is constrained by the read out from memory. For real-time knowledge editing, we seek Specifically,
%during inference Larimar's memory undergoes a fast Bayesian update -- As new data (different from training) arrives during inference,  encoding/decoding that new data in/from the memories  are postulated as Bayesian updates for which an equivalent minimization problem is leveraged. This minimization problem, which corresponds to solving a linear system of equations, is efficiently done via computing matrix pseudo inverses. This Bayesian updating mechanism of memory together with memory-augmented decoding enables Larimar to handle unseen edits in a training-free manner,  which is not the case for existing editing methods.
   

 We further exploit Larimar's memory to  enabling   generalization to long-form information beyond   the input length limit, %which is important for long horizon planning and
 which is a challenge for current LLMs. One evident way to tackle this issue is to scaling  up the input context length. An alternative path is to provide a LM decoder access to (key,value) pairs of previously seen subsequences while training the decoder on long-form text datasets. For this purpose, \citep{wu2022memorizing, wang2023augmenting}   augments the decoder with a non-differentiable memory that can store a large number of key-value pairs, query it,  and fuse retrieved key-value pairs from this module together with the in-context tokens for language modeling. 
 In contrast, we showcase here that the fixed-size, latent memory of a Larimar model which has been  trained on short sentences, can generalize to longer text by exploiting the dynamic memory update mechanism.   %can be how  leverage the dynamic updating nature of Larimar's fixed-size memory to process the long-form text during inference. %This is different from existing works that store  large number of key-value pairs in an external memory and  retrieve key value pairs to augment a layer within LLM. al  and ing, and updating storing key-value pairs which does not require . We show that  handle fact recall from long-form write in the long-form text in memory in chunks, and read out from it by querying  recursively. manner. Experiments show that Larimar is able to ha
 %\PD{add difference with existing memory-augmented transformers, in general memnets. Literarture on kanerva machines}.

% \todo{Aurelie: Finalize our key contributions once we have all experiments.}
Our contributions are: 
\begin{itemize}
    \item Inspired by complimentary learning mechanisms in brain, we propose a %Bayesian 
    memory-conditioned LLM architecture for  test time adaptation in real-time. 
    \item We demonstrate the utility of this architecture to two relevant and challenging use cases: knowledge editing and input length generalization. Larimar shows fast and accurate training-free adaptation to new inputs in both scenarios, compared to baseline editing methods and language models. 
    \item We also enable a training-free fact forgetting mechanism that exploits the %Bayesian 
    update of the memory.  %to  with a separate explicit memory module - inspired by CLS and interactions between neocortex and hippocampus
    %$\item associative memory
    %\item the memory-decoder coupling is trained such that decoder is controlled by the read/write operations corresponding to then memory
    %\item we explore both generative and deterministic memory modules
    %\item fast dynamic inference mechanism to update memory during test time -- which handles generalization better
    %\item introduce fact forgetting as a memory update operation 
    %\item speed of dynamic update
    %\item performance on new fact addition 
    %\item performance on existing fact editing benchmark 
    %\item performance on sequential and batch fact editing  
    %\item performance on fact forgetting 
    
\end{itemize}

%\begin{figure}[h]
 %   \centering
 %   \includegraphics[width=0.5\linewidth]{figures/ComplementaryLS.png}
  %  \caption{Complementary Learning System in the Human Brain}
   % \label{fig:CLS}
%\end{figure}


%Inspired by this..., we introduce Larimar -- generative LLM architectures that are coupled with generative associative memory modules.  

%In the framework, neocortex is approximated using generative LLM, whereas the memory unit represents hippocampus, former being much larger in size and complexity than later. 

%The memory unit is associative, generative, and sparsely distributed, while storing episodic memory. 

==> sections/related_work.tex <==
\section{Related Work}
\subsection{Memory-augmented NNs}

External memory augmented neural networks (MANNs) were already proposed in pre-transformer era, with the aim of better learning long-term dependencies in input data \citep{weston2014memory, graves2014neural, miller2016keyvalue}. These frameworks have shown  enhanced performance in generative tasks, language modeling,  long-term planning, and sample-efficient RL, etc. In MANNs, a trainable slot-based memory is added to a recurrent neural net. An attention-based reading mechanism is typically used to compute a weighted average of memory contents. This mechanism is estimated from training data, and thus  it remains unclear how they can generalize to new data. Alternatively, Kanerva Machine, inspired by Kanerva's sparse distributed memory model, views memory as a global latent variable in a generative model. In this framework,   the memory update and read/write are considered as Bayesian inference, i.e., the posterior parameters are updated as new data arrives. KM and its successors  show that the writing speed remains an  issue for fast updating the memory. Recently, \citep{pham2021generative}  proposed to cast memory write as a minimization problem, which provides an one-shot update mechanism for fast writing.  These conditional generative models have shown better performance on image reconstuction, denoising, and generation tasks compared to variational autoencoders and memory networks; however, to our knowledge no work is known to investigate how those models can aid in knowledge adaptation of LLMs.    .... %However, and have shown enhanced performance in generative tasks, language modeling,  long-term planning, and sample-efficient RL 

Transformers are also known to suffer from  issues such as  limited access to long-term memory and limited ability to update the memory state \citep{fan2021addressing}. One evident way to tackle this issue is to scaling up the input context length. However, recent works show that interaction between LLM’s world knowledge, embedded in its parameters, and the factual information presented in the context lacks robustness and controllability \citep{li2022large, liu2023lost}.  %An alternative path is to provide an LM decoder access to (key, value) pairs of previously seen subsequences from a non-differentiable memory while training the decoder on long-form text datasets, as proposed by  \citep{wu2022memorizing, wang2023augmenting}. 
Alternatively, transformers have been augmented with a non-differentiable long-term (or persistent) external memory,  in which  next token distributions is estimated based on not only the past context and the model parameters, but also  the retrieved  context from the external memory \citep{grave2017unbounded,khandelwal2019generalization}. %from which examples are retrieved and incorporated into the base LM’s prediction.have shown a series of impressive resultsx similar to neural cache mechanism \cite{}  has been explored to alleviate some of these issues \citep{khandelwal2019generalization,wu2022memorizing, wang2023augmenting}.  \citep{khandelwal2019generalization},   k nearest neighbors   are retrieved from an external, non-differentiable memory  storing a large number of key-value pairs and then are  fused together with the in-context tokens for better language modeling.  \citep{fan2021addressing} proposed feedback transformer, which enforces all subsequent layers attending to a memory that stores information merged from all previous layers. 
A number of works have further considered training transformers with knn-augmented attention on longer text \citep{wu2022memorizing, wang2023augmenting} and shown improved language modeling performance. 
%However, the slot-based memory modules used in these prior works struggle with scalability due to lack of distributed memory store.  Writes and reads from those slot-based memories are  difficult to scale -- as more slots need to be used for new inputs, even if they overlap with existing memories. Other models of associative memory, such as Hopfield Networks \citep{}, also face similar scalability issue, as the memory capacity remains constrained by the dimensionality of the input patterns. 
kNN-augmented LMs are further known to suffer from lack of memory control on the decoder due to the potential conflict between training-time knowledge present in model's parameters and test-time knowledge present in context, resulting in poor performance in fact update \citep{li2022large, liu2023lost, zhu2020modifying}.

In this work, we showcase for the first time how a generative memory model augmentation can enable training-free fact editing and forgetting, as well as  input length generalization of a LLM decoder.
%In contrast, Larimar's memory (i) follows a sparse distributed model, whose size  is independent from the input dimension, (ii) is generative in nature, (iii) enjoys dynamic addressing, and (iv) handles memory update via a minimization problem in inference. These properties allows fast and efficient generalization to new data without training, which we showcase in fact editing and forgetting applications, as well as in fact recall from long-form text.  %ap which allows fast adaptation to new data. These abilities provide realtime editing %  such that reading and writing weights can be fast and dynamically updated. T The goal is to achieve a  hierarchical conditional generative model,  such that (i) $M$ is a global latent variable for $X$, an episode consisting of $N$ facts, (ii) readout from $M$ is used by the decoder to reconstruct input $X$, and (iii) posterior of M can undergo fast and dynamic update by  Bayesian update. This dynamic updating mechanism of memory together with the memory-augmented decoding enables Larimar to handle unseen edits in a training-free manner,  which is not the case for existing editing methods. allowing fast memory writes and reads during inference.  and the follow-up works provides an alternative approach to this problem, in which  the memory size  is independent of the dimension of the data. 
%https://proceedings.neurips.cc/paper_files/paper/2015/file/8fb21ee7a2207526da55a679f0332de2-Paper.pdf
%Neural turing machines
%DNC
%https://arxiv.org/abs/1410.3916
%https://arxiv.org/abs/1606.03126
%feedback transformer https://arxiv.org/pdf/2002.09402.pdf
%survey paper https://dl.acm.org/doi/pdf/10.1145/3503161.3546972

\subsection{Model Editing}
Model editing seeks to make local
updates to a pre-trained base model’s behavior while satisfying three key desiderata: (i) \emph{locality}, ensuring that the model performance does not degrade elsewhere that is unrelated to edits;  (ii) \emph{generality}, ensuring that the model behaves similarly when presented with an edit reformulation; (iii) \emph{speed/scalabilty}, which is important in both sequential and batch editing situations. Numerous editing approaches have been proposed; for  comprehensive surveys on model editing methods, see \cite{yao2023editing, zhang2024comprehensive, wang2023knowledge}.   
 Editing methods broadly fall into three categories:  ''Recognition Phase", ''Association Phase' and ''Mastery Phase". ~\citep{zhang2024comprehensive}. This classification essentially accounts for whether or not the  base model's parameters are affected. ~\footnote{Note that  an alternative classification is that of ~\citep{yao2023editing} : ''Cache-based", ''Meta-learning" and ''Locate and Edit".}.  The ''recognition phase"-targeting methods consider demonstrating right context to LLMs in order to help it output correct facts, which can be achieved by in-context demonstration of similar examples from training set in \cite{IKE paper}. Alternatively, SERAC \cite{mitchell2022memory}  stores  edits in an external cache. Queries/inputs are classified whether those are within scope of the cache. If yes, a counterfactual model produces the output; if not, the input is routed to the base LLM. This class of  methods either needs multiple demonstrations retrieved from a knowledgebase or edit-specific training of scope classifier and counterfactual model.

The ''association phase" -related editing methods consider merging new knowledge to that of the base LLM, for example by either patching (adding and training) error-specific neuron, as done  in last FFN layer \cite{huang2023transformerpatcher}, or by adding  a codebook or an adaptor of  edit key-value pairs  to a specific layer, where the values are updated by using the  finetuning loss on the model’s prediction given the edit  \cite{hartvigsen2022aging}. It is worth mentioning that these two  works cited here in this category aims to handle a difficult but more realistic scenario than single fact editing - where  multiple edits are performed in a sequential manner and older edits are not forgotten.
  
  The third category of editing methods include learning to update  base LLM's own parameters. Examples are regularized finetuning \cite{} and hypernetwork-based methods \cite{Editing factual knowledge in language models; Fast model editing at scale} that often decompose weight updates into low-rank components \cite{Mend}. Recent works also explore the locate-then-edit approach, for example, references \cite{ROME, MEMIT} first perform a casual tracing to detect which part of hidden states (mostly within FFNs) can be attributable to the fact and then do a rank-one update of the corresponding weight parameters   to directly write in the updated fact (i.e., key-value pair). 

While current model editing methods have demonstrated significant  promise\citep{yao2023editing}, they do come with certain shortcomings. Existing editing methods mostly rely on either training  or  locally updating the parameters of the base model (or some auxiliary model) on an edit dataset, and generalize well  within this seen distribution. However, they are less capable of systematic generalization to edits drawn from unseen  distributions, which affects their scalability due to increased cost and speed -  issues that are critical for fixing deployed models in real-world \citep{}.   % Requirement of  edit-specific training or tracing and update, and therefore lacks generalization towards new/unrelated edits. This issue further leads to reduced speed and higher cost of edits.
 Further,  it has been reported that fact-specific knowledge within LLM is not as localized as it is believed to be \cite{hase2023does}, therefore local parameter update may not be sufficient to fully enforce the knowledge edit.  At the same time, even locally updating LLM's parameters can cause performance degradation on other tasks \cite{gu2024model}. %  they are believed to be,  leading to the leakage of information \cite{hase2023does}. On the other hand, recent works reveal that  from causal tracing methods may not correlate with edit performance \cite{hase2023does}  (iii)  
 The editing task becomes more challenging, when multiple edits are needed to be made to the model %Performance evaluation is mostly done on  when only a single edit is made to the model. It has been found that making multiple edits, 
  either in a sequential or in a batched manner, former being more realistic. Several recent works report failure of existing editing methods in those situations,  leading to significant performance degradation of the LLM (Mitchell et al., 2021, 2022; Meng et al., 2022b) \cite{gupta2024model, li2023unveiling, gu2024model}, revealing  forgetting of the older edits, causing innate knowledge distortion,  enhancing inherent knowledge inconsistencies, or loss of general abilities in LLMs. A number of external cache/memory/codebook-based editing methods have been proposed to tackle those challenges, where base model is not directly edited. However, computational efficiency in terms of writing in and reading from those slot-based memories remains to be an issue.  %Methods such as GRACE  focus on solving some of these issues \PD{how?}; however, they still require edit-specific finetuning and edits are only done at a specific layer.  %(iv) The neighborhood specificity in current editing methods appears to lack robustness \cite{hoelscher2023detecting} \PD{shall we mention as ours is no better}. 
Last but not the least, 
selective knowledge forgetting remains challenging for current model editing methods, as suggested in \cite{ishibashi2023knowledge}.\todo{Add a couple of sentences to elaborate a bit}

Our work is distinct  from existing LLM editing methods that adopt the classical view of GLM or the linear layer within as an associative memory \cite{meng2022locating} and therefore  directly update some of GLM parameters to reflect new knowledge \cite{ meng2022locating, meng2022mass}. 
Our work  is also significantly different from  model editing methods that updates a slot-based external memory %maintain an external key-value memory of fact-edit pairs and query the memory to check if the GLM needs to be updated 
\cite{han-etal-2023-improving, GRACE}, wherein  Larimar's memory is distributed and learns to compress an episode of samples in a fixed-size $M$ and therefore provides a better compression compared to slot-based memories that store key-value pairs. Further, Larimar does not need multiple demonstrations that are similar to the desired edit in order to control the decoder, as in ref \citep{zheng2023edit}. Instead,  Larimar's memory undergoes a fast training-free update as new edits arrive, which is not the case for existing editing methods. Last but not the least, the inference-time forgetting operation in Larimar is unique. %shares significant dissimilarities with that line of work, as (i) it's external memory is associative in nature: a set of $n$ facts is written in and read out from a fixed size memory,  
%Further, read out from Larimar's memory conditions the decoding to enable outputting the edit, rather than directly changing LLM parameters via training or rank-one updating. 
 % As new data (different from training) arrives during inference,  encoding new data in memories and decoding data from memories are postulated as Bayesian updates for which an equivalent minimization problem is proposed. This minimization problem, which corresponds to solving a linear system of equations, is efficiently done via computing matrix pseudo inverses. This Bayesian updating mechanism enables Larimar to handle unseen edits in a training-free manner, which is not the case for existing editing methods.

  %Previous works on generative memory models %, and more generally, associative memory models,
  %have tested model's performance mostly on image reconstruction, denoising, and generation tasks. To our knowledge, this is the first work that proposes that trains a hierarchical conditional generative memory model for language and tackle LLM editing in a more bio-inspired manner via dynamically updating the generative distributed memory.   

  \subsection{model forgetting/unlearning}
  \subsection{rag}
